RGB2Point: 3D Point Cloud Generation from Single RGB Images

We introduce RGB2Point, an unposed single-view RGB image to a 3D point cloud generation based on Transformer. RGB2Point takes an input image of an object and generates a dense 3D point cloud. Contrary to prior works based on CNN layers and diffusion denoising approaches, we use pre-trained Transformer layers that are fast and generate high-quality point clouds with consistent quality over available categories. Our generated point clouds demonstrate high quality on a real-world dataset, as evidenced by improved Chamfer distance (51.15%) and Earth Mover's distance (45.96%) metrics compared to the current state-of-the-art. Additionally, our approach shows a better quality on a synthetic dataset, achieving better Chamfer distance (39.26%), Earth Mover's distance (26.95%), and F-score (47.16%). Moreover, our method produces 63.1% more consistent high-quality results across various object categories compared to prior works. Furthermore, RGB2Point is computationally efficient, requiring only 2.3GB of VRAM to reconstruct a 3D point cloud from a single RGB image, and our implementation generates the results 15,133x faster than a SOTA diffusion-based model.

==> figures/qualitative_results/aircraft.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\columnwidth]{data/qualitative_results/aircraft.pdf}
\caption{A RGB image is reconstructed using \name is shown on the right column and the center is its ground truth.}
\label{fig:aircraft}
\end{figure}

==> rebuttal_table/ab_rebuttal_modules.tex <==
\begin{table}[ht]
    \centering
    \small
    \resizebox{0.45\textwidth}{!}{
    \begin{NiceTabular}{p{0.8cm} | p{1.2cm} p{1.2cm} | p{1.2cm} p{1.2cm} }
    \specialrule{.15em}{.05em}{.05em}
    
 \multicolumn{1}{c|}{Module} & \multicolumn{2}{c|}{ShapeNet}  & \multicolumn{2}{c}{Pix3D}\\ 
    & CD & EMD& CD & EMD  \\ 
    \midrule
    CFI& -19.27\%  & -54.43\%  & -21.86\%  & -22.73\% \\
    GPM& -31.30\%  & -55.06\%  & -26.00\%  & -41.20\% \\
    \specialrule{.15em}{.05em}{.05em}
    \end{NiceTabular}
    }
    \caption{We validated the effectiveness of our two modules by removing them from the model architecture, and we show the average of all scenes from this paper. The performances were measured using Chamfer Distance and Earth Mover's Distances. When we removed the modules CFI and GPM, the performance \textbf{dropped} compared to metrics from the original pipeline.}
    \label{tab:rebut_ablation_modules}
\end{table}

==> tables/ablation_pix3d.tex <==
\begin{table}[hbt]
    \centering
    \begin{tabular}{ccccccc}
    \specialrule{.15em}{.05em}{.05em}
      &  \multicolumn{3}{c}{Chamfer Distance} & \multicolumn{3}{c}{EMD}\\ 
    Method &Car & Chair & Aircraft & Car & Chair & Aircraft\\ 
    \midrule
    Self-Sup.~\cite{baseline} & 10.33 & 21.84 & 15.06 & 18.32 & 23.40 & 16.12\\
    Self-Sup.~\cite{baseline}+$L_{C}$ & 6.39 & 13.58 & 8.66 & 6.42 & 16.46 & 12.53\\
    Self-Sup.~\cite{baseline}+$NN$ & 5.48 & 10.91 & 7.11 & 4.95 & 14.93 & 11.07 \\
    DIFFER~\cite{differ} & 6.35 & 9.78 & 5.67 & 6.03 & 16.21 & 9.9\\
    DIFFER~\cite{differ}+$L_{G}$ & 5.63 & \underline{9.23} & \underline{5.58} & 5.35 & 13.07 & 9.44\\
    ULSP~\cite{ulsp} & 6.64 & 10.49 & 5.70 & 6.89 & 10.93 & \underline{7.43} \\
    ULSP~\cite{ulsp}+$L_{G}$ & 6.13 & 10.0 & 7.37 & 5.83 & 10.24 & 9.99 \\
    ULSP~\cite{ulsp}+Sup. & \underline{5.4} & 9.72 & 5.91 & \underline{4.78} & \underline{10.18} & 7.66 \\
    \bottomrule
    Ours & \bf{4.07} & \bf{5.02} & \bf{2.21} & \bf{3.69} & \bf{5.16} & \bf{4.38} \\
    \specialrule{.15em}{.05em}{.05em}
    \end{tabular}
    \caption{The state-of-the-art metrics from different categories in Chamfer Distance and EMD are noted in \underline{underlined}. \name\ shows an average improvement of 43.55\% in Chamfer distance and 37.72\% in Earth Movers distance.}    
    \label{tab:shapenet_table}
\end{table}
